Variational Inference of overparameterized Bayesian Neural Networks: a theoretical and empirical study

This paper studies the Variational Inference (VI) used for training Bayesian Neural Networks (BNN) in the overparameterized regime, i.e., when the number of neurons tends to infinity. More specifically, we consider overparameterized two-layer BNN and point out a critical issue in the mean-field VI training. This problem arises from the decomposition of the lower bound on the evidence (ELBO) into two terms: one corresponding to the likelihood function of the model and the second to the Kullback-Leibler (KL) divergence between the prior distribution and the variational posterior. In particular, we show both theoretically and empirically that there is a trade-off between these two terms in the overparameterized regime only when the KL is appropriately re-scaled with respect to the ratio between the the number of observations and neurons. We also illustrate our theoretical results with numerical experiments that highlight the critical choice of this ratio.

==> Proofs.tex <==
\section{Proofs}

% \subsection{Proof of \Cref{prop:F_N}}


% Since $\prior=(\priorOne)^{\otimes N}$ and $\densityq_{\btheta}(\bw) = \prod_{j=1}^N \densityq_{\theta_j}^1(w)$%, by the chain rule for the KL divergence \sm{Seems unnecesary to invoke the chain rule here, it is straightforward from the formula}
% , the first term in \eqref{eq:elbo} can be written:
% \begin{equation*}%\label{eq:elbo1}
%     \KL(\densityq_{\btheta}|\prior) = \sum_{j=1}^N \KL(\densityq_{\theta_j}|\priorOne) = N \int_{\R^{2d}} \KL(\densityq_{\theta}|\priorOne) \rmd\nu(\theta),
% \end{equation*}
%  where $\nu = \frac{1}{N} \sum_{i=1}^N \delta_{\theta_i}\in \cP(\R^{2d})$. 
 
%  We now deal with the second term of \eqref{eq:elbo}. The likelihood can be written $P(\D|\bw)=\prod_{i=1}^p P(y_i|\bw,x_i)$, 
%  and we have  assumed that $\densityq_{\btheta}=\prod_{j=1}^N \densityq_{\theta_j}=\left(\prod_{j=1}^N g(\theta_j,.)\right)_{\#}\gamma^{\otimes N}$ where $\gamma$ is the standard Gaussian distribution on $\R^d$. 
 
%  Hence, the second term in \eqref{eq:elbo} can be written:
% \begin{align*}%\label{eq:elbo2}
%     -\E_{\bw\sim \densityq_{\btheta}}[\log P(\D|\bw)]&= - \int_{\R^{N\times d}} \log P(\D|\bw)d \densityq_{\btheta}(\bw) \\
%     &= -\int_{\R^{N\times d}}\log \left(\prod_{i=1}^p \exp\left(- l( y_i, f_{\bw}(x_i)) \right)\right) \rmd\densityq_{\btheta}(\bw)\\ 
%     &= \sum_{i=1}^p \int_{\R^{N\times d}} l\left( y_i, \frac{1}{N}\sum_{j=1}^Ns(w_j, x_i)\right)\rmd\densityq_{\btheta}(\bw) \\
%  &= \sum_{i=1}^p \int_{\R^{N\times d}} l\left( y_i, \frac{1}{N}\sum_{j=1}^Ns(g(\theta_j,z_j), x_i)\right)\rmd\gamma^{\otimes N}(\bz)
%  %\\ &= \sum_{i=1}^p \int_{\R^d} l\left( y_i, \int_{\R^{2d}} s(g(\theta,z), x_i) d\nu(\theta)\right)d\gamma(z) 
% \end{align*}
% where the last equality uses the transfer lemma $\int_{\R^{N\times d}} F\circ T(\bz) \rmd\gamma^{\otimes N}(\bz)=\int_{\R^{N\times d}} F(\bw)\rmdT_{\#}\gamma(\bw)$ for any bounded and measurable function $F$, where $T = \prod_{j=1}^N g(\theta_j,.): \R^{N\times d} \to \R^{N\times d}$.\ak{justify exchangeability and reparametrization by $\nu_N$}
%uses the change of variable $w=g(\theta,z)=\mu +\sigma z$, where $|dw/dz|=\prod_{k=1}^d\sigma_k$, that cancels with the same term in the normalization constant of $\gamma$.
%Rescaling the two terms by $1/N$ yields the result.




%\begin{lemma}\label{lem:reparametrization}
%Let $f_N$ defined for any $\rho \in \R$ by:
%\begin{equation*}
 %   f_N(\rho) = \frac{-\sqrt{N}}{ch(N(\rho-\log(e^{\tau}-1))}) + \sqrt{\frac{\tau^2}{2} \left[ \log\left(\frac{\tau^2}{\log(e^{\rho}+1)^2}\right) + \frac{\log(e^{\rho}+1)^2}{\tau^2} - 1\right]}
%\end{equation*}
%This reparametrization verifies:
%\begin{enumerate}
%    \item $\lim\limits_{N \rightarrow +\infty} f_N(\rho) = c$ in $V_2$ defined in \eqref{eq:V_2},
%    \item $f_N(\rho): \R \rightarrow ]-\frac{\tau\sqrt{N}}{\sqrt{\alpha p}}, +\infty[$ 
%    \item $\alpha V_1(\theta) = \frac{V_2(\theta)}{p}$ 
%\end{enumerate}
%\end{lemma}

%\begin{proof}
%\sm{Some reminder of definition of $f_{\infty}$ would be apropriate here. As well as a sentence that explains why the first term disappears when $N \rightarrow \infty$.}
%1. For any $\rho \in \R$, $\lim\limits_{N \rightarrow +\infty} f_N(\rho) = f_{\infty}(\rho)=c$.\\

%2. Notice that $f_{\infty}(\rho)=\sqrt{\tau^2 \KL(p|q)}$ where $p \sim N(0, \tau^2)$ and $q \sim N(0, \log(e^{\rho}+1)^2)$; hence $f_{\infty}(\rho)\ge 0$ with equality when the distributions are equals ($\tau = \log(e^{\rho}+1)$). The first term of $f_N(\rho)$ is also minimal when $\rho = \log(e^{\tau}-1)$, and in this case the minimum is $-\frac{\tau\sqrt{N}}{\sqrt{\alpha p}}$. \\

%3.  Since $f_N(\rho) = f_{\infty}(\rho) + o(1)$, we can write 
%\begin{equation}
 %   \begin{split}
  %      \frac{V_2(\theta)}{p} = \sum_{k=1}^{d}{\frac{f_{\infty}(\rho)^2 \alpha }{\tau_k^2}+ \frac{\alpha(\mu_k - \mu_k')^2}{2\tau_k^2}}
 %       = \sum_{k=1}^{d}{\frac{\frac{\tau^2}{2} \left[ \log(\frac{\tau^2}{\log(e^{\rho}+1)^2}) + \frac{\log(e^{\rho}+1)^2}{\tau^2} - 1\right] \alpha }{\tau_k^2}+ \frac{\alpha(\mu_k - \mu_k')^2}{2\tau_k^2}} \\
 %        =\frac{\alpha}{2}\sum_{k=1}^{d}{\log(\frac{\tau^2}{\log(e^{\rho}+1)^2}) + \frac{\log(e^{\rho}+1)^2}{\tau^2} - 1 + \frac{(\mu_k - \mu_k')^2}{\tau_k^2}} 
 %        = \alpha V_1(\theta).
 %   \end{split}\qedhere
%\end{equation}
%\end{proof}
\subsection{Proof of \Cref{prop:non_asymptotic_bound}}



\begin{proof}

Let $\nu^N=\nicefrac{1}{N}\sum_{j=1}^N \updelta_{\theta_j}$. We recall the notation $\bz=(z_1,\dots,z_N)\in \R^{N\times d}$. Let 
\begin{equation*}
    A_N^i(\bz)=\frac{1}{N}\sum_{j=1}^N \phi(\theta_j, z_j, x_i),\quad B_N^i= \iint_{\R^{2d}\times \R^d} \phi(\theta,z,x_i)\rmd\nu^N(\theta)\rmd\gamma(z),\quad D_N^i(\bz)= A_N^i(\bz)-B_N^i.
\end{equation*}
Since $z_1,\dots,z_N$ are i.i.d. as $\gamma$, we first have
\begin{align*}
\E_{\bz \sim \gamma^{\otimes N}}[D_N^i(\bz)]&= \E_{\bz \sim \gamma^{\otimes N}}[A_N^i(\bz)] -B_N^i= \frac{1}{N}\sum_{j=1}^N\int_{\R^d} \phi(\theta_j,z,x_i)\rmd \gamma(z) - B_N^i= 0,\\
\Var_{\bz\sim \gamma^{\otimes N}}(D_N^i(\bz))&=\Var_{\bz\sim \gamma^{\otimes N}}(A_N^i(\bz))=\frac{1}{N^2} \sum_{j=1}^N \Var_{z\sim  \gamma}(\phi(\theta_j, z,x_i))=\frac{1}{N}\int_{\R^{2d}}\Var_{z\sim  \gamma}(\phi(\theta, z,x_i))d\nu^N(\theta)\\
&\le \frac{1}{N^2}\sum_{j=1}^N \E_{z\sim \gamma}\left[\|\phi(\theta_j,z,x_i\|^2 \right]\le \frac{1}{N^2}\sum_{j=1}^N c_{\phi} \E_{z\sim\gamma}\left[(1+\|z\|)^2\right]\|\theta\|^2\|x_i\|^2 \le \frac{C^2}{N},
\end{align*}
under \Cref{ass:activation_function} and assuming the $\theta$'s are in a compact  set of $\R^{2d}$\ak{need more justifications/details here.} \ak{check the bound on the variance. the $x_i$ disappears if we consider bounded activation functions}.
We can also upper bound, 
\begin{equation*}
|\E_{\bz \sim \gamma^{\otimes N}}[D_N^i(\bz)]|\le \E_{\bz \sim \gamma^{\otimes N}}[|D_N^i(\bz)|]\le \sqrt{\E_{\bz \sim \gamma^{\otimes N}}[(D_N^i(\bz))^2]}=\sqrt{\Var_{\bz \sim \gamma^{\otimes N}}(D_N^i(\bz))}\le \frac{C}{\sqrt{N}}.
\end{equation*}


We have:
\begin{multline*}
\left\vert\rmG^{N,p}(\nu^N) - \hat{\rmG}^p(\nu^N)\right\vert
 =  \left\vert \sum_{i=1}^p\left( \E_{\bz\sim \gamma^{\otimes N}} \left[l\left( y_i, 
A_N^i(\bz)
 \right)\right] -  l\left(y_i, B_N^i\right)\right)\right\vert
=  \left\vert \sum_{i=1}^p  \E_{\bz\sim \gamma^{\otimes N}} \left[ l\left( y_i, 
D_N^i(\bz)
 \right) - l\left(y_i, B_N^i\right) \right] \right\vert,
\end{multline*}
since the second term in the expectation is a constant.


For a loss satisfying \Cref{ass:lipschitz_loss}, 
\begin{equation*}
    \left\vert l\left(y_i,A_N^i(\bz) \right) - l\left(y_i, B_N^i\right)\right \vert 
    \leq L(y_i) D_N^i(\bz).
\end{equation*}
Hence, we have
\begin{equation*}
    \left\vert\rmG^{N,p}(\nu^N) - \hat{\rmG}^p(\nu^N)\right\vert\le \sum_{i=1}^p  L(y_i)\E_{\bz\sim \gamma^{\otimes N}}\left[ D_N^i(\bz)\right]  \le  \left\vert\sum_{i=1}^p  L(y_i) \right\vert \frac{C}{ \sqrt{N}}.
\end{equation*}

Under \Cref{ass:square_loss}, i.e. for the square loss,
\begin{equation*}
    \sum_{i=1}^p \E_{\bz\sim\gamma^{\otimes N}}\left[ l\left(y_i, A_N ^i(\bz) \right)\right]= \sum_{i=1}^p \|y_i\|^2 +2 \sum_{i=1}^p\E_{\bz\sim \gamma^{\otimes N}}\left[ \ps{y_i,A_N ^i(\bz)}\right] + \sum_{i=1}^p \E_{\bz\sim \gamma^{\otimes N}}\left[ \|A_N^i(\bz)\|^2\right].
\end{equation*}
First, by marginalizing over $\gamma^{\otimes N}$,
\begin{equation*}
 \sum_{i=1}^p\E_{\bz\sim \gamma^{\otimes N}}\left[ \ps{y_i,A_N ^i(\bz)}\right]  = \sum_{i=1}^p     \ps{y_i,\E_{\bz \sim \gamma^{\otimes N}}\left[A_N^i(\bz)\right]} 
=\sum_{i=1}^p \ps{y_i,B_N^i}.% = \sum_{i=1}^p \iint_{\R^{d}\times \R^{2d}}\ps{y_i, \phi(\theta,z,x_i)}\rmd\gamma(z)\rmd\nu^N(\theta). 
\end{equation*}
Then,
\begin{multline*}
 \sum_{i=1}^p \E_{\bz\sim \gamma^{\otimes N}}\left[ \|A_N^i(\bz)\|^2\right] = \sum_{i=1}^p  \left( \Var_{\bz\sim \gamma^{\otimes N}}(A_N^i(\bz)) + \|\E_{\bz \sim \gamma^{\otimes N}}\left[A_N^i(\bz)\right]\|^2 \right)\\
 =\sum_{i=1}^p\frac{1}{N}\int_{\R^{2d}} \Var_{z\sim  \gamma}(\phi(\theta, z,x_i))d\nu^N(\theta) +\left\Vert B_N^i \right\Vert^2.
 %\left\Vert \int_{\R^{2d}}\phi(\theta,z,x_i)d\nu^N(\theta)d\gamma(z) \right\Vert^2.
\end{multline*}
Hence, 
\begin{equation*}
    \left\vert\rmG^{N,p}(\nu^N) - \hat{\rmG}^p(\nu^N)\right\vert =\left\vert \sum_{i=1}^p \frac{1}{N}\int_{\R^{2d}} \Var_{z\sim  \gamma}(\phi(\theta, z,x_i))d\nu^N(\theta) 
    \right\vert \le \sum_{i=1}^p \frac{C^2}{N}.
\end{equation*}
\ak{we get N instead of $\sqrt{N}$ for the square loss}
\end{proof}



\subsection{Proof of \Cref{prop:limiting_functional}}

\begin{proof}
%Sketch of proof:
%\begin{enumerate}
%    \item use \Cref{prop:non_asymptotic_bound} :
%    $|\rmG^{p,N}(\nu^N) - \hat{\rmG}^{p}(\nu^N)|\le \frac{C_p}{\sqrt{N}}$
%    \item use pointwise convergence of $\hat{\rmG}=\frac{1}{p}\hat{\rmG}^p $ to $\rmG$ so $\hat{\rmG}(\nu^N) \to \rmG(\nu^N)$ 
%    \item use $|\rmG(\nu^N) - \rmG(\nu)|\to 0$ for $\nu^N\to \nu$ (W2 cv)
%\end{enumerate}
%1+2+3 gives $\rmG^{p,N}(\nu^N) \to \rmG(\nu)$.

%\sm{I don't think the above will work. 2+3 alone don't give the convergence we want. The way to show it is:}
%\begin{enumerate}
%    \item use \Cref{prop:non_asymptotic_bound}
%    \item show a bound for $\| \hat{\rmG}^{p}(\nu_N) - G^p(\nu) \|$, in a way analogous to \Cref{prop:non_asymptotic_bound}
%    \item show pointwise convergence of $G^p(\nu)$ to $G(\nu)$.
%\end{enumerate}
We will first derive a bound for $| \hat{\rmG}^{p}(\nu_N) - \rmG^p(\nu) |$.
We denote $H^i = \int \phi(\theta, z, x_i) d\nu(\theta)d\gamma(z)$. By \Cref{ass:activation_function} \sm{we will need that}, we have that $\theta \mapsto \int \phi(\theta, z, x_i) d\gamma(z)$ is Lipschitz continuous with constant $C_0 + C_1\norm{x_i}$ on the compact set to which $\theta$ belong. Since $\nu^N$ are compactly supported and converge weakly to $\nu$, they converge in $W_1$ distance.

Under \Cref{ass:lipschitz_loss}, we get:
\begin{equation*}
    \verts{l(y_i, B_N^i) - l(y_i, H_i)} \leq L(y_i) \verts{B_N^i - H_i} \leq W_1(\nu^N, \nu) (C_0 + C_1\norm{x_i})
\end{equation*}
Combining the above bound with the one from \Cref{prop:non_asymptotic_bound}, we get:
\begin{equation*}
    \verts{\frac{1}{p}\rmG^{N,p}(\nu^N) - \frac{1}{p} \sum_{i=1}^p l(y_i, H_i)} \leq \frac{C}{\sqrt{N}} \left(\frac{\sum_{i=1}^p L(y_i)}{p}\right) + W_1(\nu^N, \nu) \frac{1}{p}\sum_{i=1}^p (C_0 + C_1\norm{x_i}).
\end{equation*}
Therefore, provided that the data distribution $\pi$ has finite first moment:
\begin{equation*}
    \lim_{N,p \rightarrow \infty}  \rmG^{N,p}(\nu^N) = \lim_{N,p \rightarrow \infty} \frac{1}{p} \sum_{i=1}^{p} l(y_i, H_i)=\rmG(\nu).
\end{equation*}
To get the final limit, we need a condition that assures that $l(y_i, H_i)$ has finite expectation and use law of large numbers. 
%Choose a given $y^*$ and $\theta^*$ in the compact support of $\nu$. Denote $H_i^* = \int \phi(\theta^*, z, x_i) d\gamma(z)$. 
We have, since $l(y_i,y_i)=0$:
\begin{equation*}
\verts{l(y_i,H_i)} =   \verts{l(y_i, H_i) - l(y_i, y_i)} \leq L(y_i) \verts{y_i - H_i} \leq L(y_i)\verts{y_i} + L(y_i)\verts{H_i}
\end{equation*}

%\sm{Maybe we need to assume that $l(y,y)$ is bounded? Or a constant?}\ak{we will always have $l(y,y)=0$}

...

For the square loss, we have:
\begin{align*}
    \verts{l(y_i, B_N^i) - l(y_i, H_i)} & = \verts{2y_i(H_i - B_N^i) + (B_N^i)^2 - H_i^2}  \leq \verts{2y_i + H_i + B_N^i} \verts{B_N^i - H_i} \\
    & \leq \verts{2y_i + H_i + B_N^i} W_1(\nu_N, \nu) (C_0 + C_1 \norm{x_i})
\end{align*}
Combining the above bound with the one from \Cref{prop:non_asymptotic_bound}, we get:
\begin{equation*}
    \verts{\frac{1}{p}\rmG^{N,p}(\nu_N) - \frac{1}{p} \sum_{i=1}^p l(y_i, H_i)} \leq \frac{C}{\sqrt{N}} \left(\frac{\sum L(y_i)}{p}\right) + W_1(\nu_N, \nu) \frac{1}{p}\sum_{i=1}^p (C_0 + C_1\norm{x_i}).
\end{equation*}
\end{proof}

\subsection{Wasserstein space topology background and introductory lemmas}\label{sec:introductory_lemmas}
%\ak{also, $W_2$ cv implies $W_1$ cv which implies weak convergence \citet[Proposition 7.1.5]{ambrosio2008gradient}}

In this subsection we review results about the  topology of Wasserstein spaces that are relevant to our proof for  Gamma convergence in  \Cref{sec:proof_gamma_gonv}. We denote by $W_p$ the p-Wasserstein space.  
\Cref{lem:shifting_potential_weak_convergence} will be useful to prove the upper bound \eqref{eq:upp_bound_gamma}. Then, \Cref{th:villani} and \Cref{lem:shifting_potential_convergence} will be useful to show \eqref{eq:eq_bound_gamma}. \Cref{lem:rescaling_functionals} will be useful to rescale $\rmF^N$ to yield $\tilde{\rmF}_i^N(\nu)$, $i=1,2$.


In order to prove convergence of minimizers using \Cref{th:gamma_conv}, we will need to find compact subsets of $W_2$ containing minimizers the family of functionals $\rmF^N$ considered in \Cref{sec:gamma_conv}. The following characterization of precompact sets in $W_p$ spaces will be useful.


\begin{theorem}\citet[Theorem 7.12] {villani2003topics} \label{th:villani} 
Let $(\nu^N)_{N\in \N^*}$ be a sequence of probability measures in $\cP(\R^d)$ and $\nu \in \cP(\R^d)$. Then, the following are equivalent:
\begin{itemize}
    \item (i) $W_p(\nu^N,\nu)\to0$;
    \item (ii) $\nu^N\to \nu$ weakly and $\int\|x\|d\nu^N(x)\to \int \|x\|d\nu(x)$;
    \item (iii) $\nu^N\to \nu$ weakly and $\sup_{N} \int_{x , \norm{x} > R} \norm{x}^p d\nu^N(dx) = 0$;
    \item (iv) for any $C>0$ and continuous $\phi: \R^d \rightarrow \R^+$ such that $\phi(x) \leq C(1 + \norm{x - x}_2^p)$ for all $x\in \R^d$, $\int f(x)d\nu^N(x)\to \int f(x)d\nu(x)$.
\end{itemize}
%Assume that for some continuous $\phi: \R^d \rightarrow \R^+$ we have $\phi(x) \leq C_1\norm{x - x_0}_2^2 + C_2$ for some $x_0 \in \R^d$ and $C_1,C_2 \in \R^{+}$. Then $\lim_{N \rightarrow \infty} \int \phi(x) \nu^N(dx) = \int \phi(x) \nu(dx)$.
\end{theorem}

%\ak{see Prkhorov}\ak{à virer}
\begin{proposition}\citet[Proposition 2.2.3]{panaretos2020invitation} \label{thm:wassersteinprecompactness}
    A weakly tight set of measures $K \subset W_p(\R^d)$ is precompact in Wasserstein space if and only if
    \begin{equation}\label{eq:characterization_compact}
        \lim_{R \rightarrow \infty} \sup_{\mu \in K} \int_{x , \norm{x} > R} \norm{x}^p \mu(dx) = 0.
    \end{equation}
\end{proposition}

\begin{proof}
Suppose that \Cref{eq:characterization_compact} holds. If $\nu^N \in K$, then there
exists a measure $\nu_0$ such that $\nu^N\to\nu_0$ weakly (up to a subsequence), and as \Cref{th:villani}-(iii)
holds for that subsequence, it converges in the Wasserstein space.
Conversely, if \eqref{eq:characterization_compact} does not hold, then we can find a sequence $\nu^N \in K$ such that
for some $\epsilon>0$, for all $N\in \N^*$, $\int$
Obviously no subsequence of $\nu^N$ can converge in the Wasserstein space, in view of
\Cref{th:villani}-(iii). Thus $K$ is not compact in $W_p$.
\end{proof}


\begin{comment}
\begin{lemma}
Let $V^N : \R^d \rightarrow \R$ be a sequence of nonnegative continuous functions, that converge pointwise to a function $V$, uniformly on compact sets. Let $\nu^N$ be a sequence of probability measures on $\R^d$ converging weakly to a probability measure $\nu$. Then we have:
\begin{equation*}
    \liminf_{N \rightarrow \infty} \int V^N(x) \nu_N(dx) \geq \int V(x) \nu(dx)
\end{equation*}
\end{lemma}
\begin{proof}
For a given $R >0$, we define the following fun $\phi_R(x): \R^m \rightarrow [0,1]$ to be a continuous approximation of the characteristic function of the ball $B(0,R)$, defined by:
\begin{equation*}
    \phi_R(x) = 
    \left\{
    \begin{array}{ll}
		1  & \mbox{if } \norm{x} \leq R \\
		R + 1 - \norm{x} & \mbox{if } R < \norm{x} < R+1 \\
		0 & \mbox{if } \norm{x} \geq R +1
	\end{array}
	\right.
\end{equation*}
Choose an arbitrary $\epsilon > 0$ and $R > 0$. We have:
\begin{equation*}
    \liminf_{N \rightarrow \infty} \int V^N(x) \nu_N(dx) \geq \liminf_{N \rightarrow \infty} \int V^N(x) \phi_R(x) \nu_N(dx).
\end{equation*}
By assumption of uniform convergence of $V^N$ to $V$ on compact sets, we know that for big enough $N$ we have $\sup_{\norm{x} \leq R+1} \vert V^N(x) - V(x) \vert \leq \epsilon$. Therefore
\begin{equation*}
    \liminf_{N \rightarrow \infty} \int V^N(x) \phi_R(x) \nu_N(dx)  \geq \liminf_{N \rightarrow \infty} \int V(x) \phi_R \nu_N(dx) - \epsilon = \int V(x) \phi_R(x) \nu(dx) - \epsilon.
\end{equation*}
%where the equality is a consequence of the fact that $V(x)\phi_R(x)$ is a continuous bounded function and $\nu_N$ converges weakly to $\nu$.
Since the above holds for all $\epsilon, R > 0$, it follows that:
\begin{equation*}
     \liminf_{N \rightarrow \infty} \int V^N(x) \nu_N(dx) \geq \lim_{R \rightarrow \infty} \int V(x) \phi_R(x) \nu(dx) = \int V(x) \nu(dx)
\end{equation*}
which concludes the proof.
\end{proof}
\end{comment}
%\begin{lemma}
%Let $V^N(x_1, x_2) : \R^d \times \R^d \rightarrow \R$ be a sequence of continuous, positive-semidefinite functions such that converge pointwise to a positive semidefinite function $V : \R^d \times \R^d \rightarrow \R$.
%\end{lemma}
\begin{lemma} \label{lem:shifting_potential_weak_convergence}
Let $V^N : \R^d \rightarrow \R$ be a sequence of continuous functions, that converge pointwise to a function $V$, uniformly on compact sets. Let $\nu^N$ be a sequence of probability measures on $\R^d$ converging weakly to a probability measure $\nu$. Assume that there exists a nonnegative function $g: \R^d \rightarrow \R$ such that $V^N + g \geq 0$ for all $N \in \N$ and $\limsup_{N \rightarrow \infty} \int g(x) \nu^N(dx) \leq \int g(x) \nu(dx)$. Then we have:
\begin{equation*}
    \liminf_{N \rightarrow \infty} \int V^N(x) \nu^N(dx) \geq \int V(x) \nu(dx)
\end{equation*}
\end{lemma}
\begin{proof}
By assumption, the functions $U^N(x) = V^N(x) + g(x)$ are nonnegative and converge to a function $U = V + g$ uniformly on compact sets. For a given $R >0$, we define the following fun $\phi_R(x): \R^m \rightarrow [0,1]$ to be a continuous approximation of the characteristic function of the ball $B(0,R)$, defined by:
\begin{equation*}
    \phi_R(x) = 
    \left\{
    \begin{array}{ll}
		1  & \mbox{if } \norm{x} \leq R \\
		R + 1 - \norm{x} & \mbox{if } R < \norm{x} < R+1 \\
		0 & \mbox{if } \norm{x} \geq R +1
	\end{array}
	\right.
\end{equation*}
Choose an arbitrary $\epsilon > 0$ and $R > 0$. We have:
\begin{equation*}
    \liminf_{N \rightarrow \infty} \int U^N(x) \nu^N(dx) \geq \liminf_{N \rightarrow \infty} \int U^N(x) \phi_R(x) \nu^N(dx).
\end{equation*}
Since $U^N$ converge to $U$ uniformly on compact sets, we know that for big enough $N$ we have $\sup_{\norm{x} \leq R+1} \vert U^N(x) - U(x) \vert \leq \epsilon$. Therefore
\begin{equation*}
    \liminf_{N \rightarrow \infty} \int U^N(x) \phi_R(x) \nu^N(dx)  \geq \liminf_{N \rightarrow \infty} \int U(x) \phi_R \nu^N(dx) - \epsilon = \int U(x) \phi_R(x) \nu(dx) - \epsilon.
\end{equation*}
Since the above holds for all $\epsilon, R > 0$, it follows that:
\begin{equation} \label{eq:shifting_potential_weak_conv}
     \liminf_{N \rightarrow \infty} \int U^N(x) \nu^N(dx) \geq \lim_{R \rightarrow \infty} \int U(x) \phi_R(x) \nu(dx) = \int U(x) \nu(dx).
\end{equation}
For any sequences of real numbers $(a_N)_{N\in \N^*}, (b_N)_{N\in \N^*}$ we have:
\begin{equation*}
     \liminf_{N \rightarrow \infty} a_N + \limsup_{N \rightarrow \infty} b_N \geq \liminf_{N \rightarrow \infty} a_N + b_N
\end{equation*}
which follows from the trivial inequality $\liminf_{N \rightarrow \infty} \tilde{a}_N + \tilde{b}_N  \geq \liminf_{N \rightarrow \infty} \tilde{a}_N + \liminf_{N \rightarrow \infty} \tilde{b}_N$ by taking $\tilde{a}_N = a_N + b_N, \tilde{b}_N = -b_N$, reorganizing the terms and using $\liminf_{N \rightarrow \infty} - b_N = - \limsup_{N \rightarrow \infty} b_N$. Using those inequalities and \ref{eq:shifting_potential_weak_conv}, we obtain:
\begin{align*}
     \liminf_{N \rightarrow \infty} \int V^N(x) \nu^N(dx) + \limsup_{N \rightarrow \infty} \int g(x) \nu^N(dx) & \geq \liminf_{N \rightarrow \infty} \int U^N(x) \nu^N(dx) \\ & \geq \int U(x) \nu(dx) = \int V(x) \nu(dx) + \int g(x) \nu(dx).
\end{align*}
By assumption $\limsup_{N \rightarrow \infty} \int g(x) \nu^N(dx) \leq \int g(x) \nu(dx)$, we now obtain the thesis.
\end{proof}
The following will be a useful corollary to lemma \ref{lem:shifting_potential_weak_convergence}:

\begin{corollary}\label{lem:shifting_potential_convergence}
Let $V^N : \R^d \rightarrow \R$ be a sequence of continuous functions such that $\lim_{N \rightarrow \infty} V^N(x) = V(x)$, uniformly on compact sets. Suppose that $\sup_{N \in \N^*} \verts{V^N(x)} \leq C_0 + C_1 \norm{x}^s$ for some $C_0, C_1 \geq 0$, and $s \in \{1,2\}$. Let $(\nu^N)_{N\in \N^*}$ be a sequence of measures in $\cP(\R^d)$ such that $\lim_{N \rightarrow \infty} W_s(\nu^N, \nu) = 0$ for some $\nu \in \cP(\R^d)$. Then:
\begin{equation*}
    \lim_{N \rightarrow \infty} \int_{\R^d} V^N(x) \nu^N(dx) = \int V(x) \nu(dx).
\end{equation*}
\end{corollary}
\begin{proof}
Since $\nu_N$ converges to $\nu$ in $W_s$ distance, it converges weakly and $\lim_{N \rightarrow \infty} \int C_0  + C_1 \norm{x}^s \nu_N(dx) = \int C_0 + C_1 \norm{x}_2^2 \nu(dx)$. We also have $V^N(x) + C_0 + C_1\norm{x}^s \geq 0$ and $-V^N(x) + C_0 + C_1\norm{x}^s \geq 0$ for all $N \in \N^*, x \in \R^d$. Therefore, by \ref{lem:shifting_potential_weak_convergence} we get:
\begin{align*}
    \liminf_{N \rightarrow \infty} \int V^N(x) \nu^N(dx) \geq \int V(x) \nu(dx)\quad \text{ and }\quad
    \liminf_{N \rightarrow \infty} \int - V^N(x) \nu^N(dx) & \geq \int -V(x) \nu(dx).
\end{align*}
Using $\liminf_{N \rightarrow \infty} - a_N =  -\limsup_{N\rightarrow \infty} a_N$, we now get:
\begin{equation*}
    \int V(x) \nu(dx) \geq  \limsup_{N \rightarrow \infty} \int V^N(x) \nu^N(dx) \geq  \liminf_{N \rightarrow \infty} \int V^N(x) \nu^N(dx) \geq \int V(x) \nu(dx),
\end{equation*}
from which the thesis follows.
\end{proof}

\begin{comment}
\begin{lemma}
Let $V^N : \R^d \rightarrow \R$ be a sequence of continuous functions such that $\sup_{N \in \N^*} \verts{V^N(x)} \leq C_1 \norm{x}_2^2 + C_2$ for some $C_1, C_2 \geq 0$, and $\lim_{N \rightarrow \infty} V^N(x) = V(x)$, uniformly on compact sets. Let $(\nu^N)_{N\in \N^*}$ be a sequence of measures in $\cP(\R^d)$ such that $\lim_{N \rightarrow \infty} W_2(\nu^N, \nu) = 0$ for some $\nu \in \cP(\R^d)$. Then:
\begin{equation*}
    \lim_{N \rightarrow \infty} \int_{\R^d} V^N(x) \nu^N(dx) = \int V(x) \nu(dx).
\end{equation*}
\end{lemma}

\begin{proof}
Denote $A = \{\nu^N\}_{N=1}^{\infty} \cup \{\nu\}$. Since the sequence $\nu^N$ converges to $\nu$ in the $W_2$ sense, the set $A$ is precompact in $W_2$ topology. Choose an $\epsilon > 0$. By characterization \Cref{thm:wassersteinprecompactness}, there exists $R(\epsilon) > 0$ such that:
\begin{equation}\label{eq:sup_out_compact}
 \sup_{\mu \in A} \int_{x : \norm{x}_2 > R(\epsilon)} (C_1 \norm{x}_2^2 + C_2) \mu(dx) < \frac{\epsilon}{4}.
\end{equation} 
Note that since $V^N$ converges pointwise to $V$, we also have $\vert V(x) \vert \leq C_1\norm{x}_2^2 + C_2$ for any $x$ \ak{in $\left\{x : \norm{x}_2 > R(\epsilon)\right\}$?}. From this and \eqref{eq:sup_out_compact}, we can conclude
\begin{equation*}
    \left\vert \int_{x : \norm{x}_2 > R(\epsilon)} V^N(x) \nu^N(dx) -  \int_{x : \norm{x}_2 > R(\epsilon)} V(x) \nu^N(dx) \right\vert  \leq \int_{x : \norm{x}_2 > R(\epsilon)} \left\vert V^N(x) - V(x) \right\vert \nu^N(dx) < \frac{\epsilon}{2}.
\end{equation*}
Furthermore, since $V^N(x)$ converges to $V(x)$ uniformly on compact sets, we know that there exists $k \in \N$
such that for $N >k$ we have $\sup_{\norm{x}_2 \leq R(\epsilon)} \verts{V^N(x) - V(x)} < \frac{\epsilon}{2}$. Therefore, for $N > k$
\begin{equation*}
    \left\vert \int_{x : \norm{x}_2 \leq R(\epsilon)} V^N(x) \nu^N(dx) - \int_{x : \norm{x}_2 \leq R(\epsilon)} V(x) \nu^N(dx) \right\vert < \frac{\epsilon}{2}.
\end{equation*}
The above bounds imply, that for $N > k$ we have
\begin{equation*}
    \left\vert \int V^N(x)\nu^N(dx) - \int V(x) \nu^N(dx) \right\vert < \epsilon,
\end{equation*}
and therefore
\begin{align*}
    \liminf_{N \rightarrow \infty} \int V^N(x)\nu^N(dx) & \geq \liminf_{N \rightarrow \infty} \int V(x) \nu^N(dx) - \epsilon \\
    \limsup_{N \rightarrow \infty} \int V^N(x) \nu^N(dx) & \leq \limsup_{N \rightarrow \infty} \int V(x) \nu^N(dx) + \epsilon
\end{align*}
for any $\epsilon > 0$. From this we infer
\begin{equation*}
    \liminf_{N \rightarrow \infty} \int V(x) \nu^N(dx) \leq  \liminf_{N \rightarrow \infty} \int V^N(x)\nu^N(dx) \leq \limsup_{N \rightarrow \infty} \int V^N(x) \nu^N(dx) \leq \limsup_{N \rightarrow \infty} \int V(x) \nu^N(dx).
\end{equation*}
Now, by \Cref{th:villani} we have $\lim_{N \rightarrow \infty} \int V(x)\nu^N(dx) = \int V(x) \nu(dx)$. Together with the above inequalities, this implies the thesis.
\end{proof}
\end{comment}

In order to verify the conditions of \Cref{lem:shifting_potential_convergence}, we will use the following result.
\begin{lemma} \label{lem:uniform_convergence_from_uniform_Lsmoothness}
Let $V^N(x) : \R^d \rightarrow \R$ be a sequence of $C^1$ functions, such that the gradient of $V^N(x)$ is $L_N$-Lipschitz. Assume that $(V^N)_{N\in \N}$ converges pointwise to $V$, and that $\sup_{N} L_N \leq L < \infty$. Then $(V^N)_{N \in \N}$ converges to $V$ uniformly on compact sets. Furthermore, there exists $C_1, C_2$ such that $\sup_{N \in \N} \verts{V^N(x)} \leq C_1 \norm{x}^2 + C_2$, and thus conditions of \ref{lem:shifting_potential_convergence} are satisfied.
\end{lemma}
\begin{proof}
For convenience, we will show that $V^N$ converge to $V$ uniformly on all closed balls $\overline{B}(0, R) = \{ x : \norm{x}_2 \leq R\}$. This of course implies uniform convergence on all compact sets. Choose $r >0$. We start by showing, that the family of functions $(V^N)_{N\in \N^*}$ is uniformly Lispchitz continuous on $\overline{B}(0,R)$.

Let $y_0 = 0$ and $y_i = e_i \cdot R$ for $i \in \{1, \ldots, d \}$, that is $y_i$ is a point in $\R^d$ with $i$-th coordinate equal to $R$ and all other coordinates equal to $0$. Since $V_N$ converge to $V$ pointwise, there exists $k \in \N$ such that for all $N >k$ and $i \in \{0,1, \ldots, d\}$ we have $\vert V^N(y_i) - V(y_i) \vert < \frac{1}{2}$. Assume from now that $N > K$. By the mean value theorem, for all $1 \leq i \leq d$ there exists $z_i$ on the segment $(y_0, y_i)$ such that
\begin{equation*}
    \frac{\partial}{\partial x_i} V^N(z_i) = \frac{V^N(y_i) - V^N(y_0)}{R} \leq \frac{V(y_i) - V(y_0) + 1}{R}.
\end{equation*}
Since gradients of $V^N$ are $L$-Lipschitz, we have 
\begin{equation*}
\verts{\frac{\partial}{\partial x_i} V^N(y_0)} \leq  \verts{\frac{\partial}{\partial x_i} V^N(z_i)} + L\norm{z_i - y_0}_2 \leq \verts{\frac{V(y_i) - V(y_0) + 1}{R}} + LR.
\end{equation*}
The above inequality implies, that $\norm{\nabla V^N(y_0)}$ is uniformly bounded for $N > k$, and therefore it is uniformly bounded for all $N \in \N$. This implies, that $\sup_{N \in \N} \sup_{x \in \overline{B}(0,R)} \norm{\nabla V^N(x)} < + \infty$.
Since $\{V^N\}_{N=1}^{\infty}$ is a uniformly Lipschitz continuous family of functions, it is equicontinuous. We will now argue that $V^n$ converge to $V$ uniformly by contradiction. Suppose that $V^N$ do not converge uniformly to $V$. Then there is a subsequence $V^{N_m}$ such that $\limsup_{m \rightarrow \infty} \sup_{x \in \overline{B}(0,R)} \verts{V^{N_m}(x) - V(x)} > 0$. But by Arzela-Ascoli theorem, there is a further subsequence of $V^{N_m}$ that converges uniformly \ak{on $\overline{B}(0,R)$ right}, and the only possible limit of that subsequence is $V$. This is a contradiction, and therefore $V^N$ converge to $V$ uniformly \ak{on closed balls.}.

To prove the second part of the lemma, we first use the $L$-smoothness inequality:
\begin{align*}
    \verts{V^N(x)} & \leq \verts{V^N(0)} + \langle \nabla V^N(0), x \rangle + \frac{L}{2} \norm{x}^2 
    \leq \verts{V^N(0)} + \frac{\norm{\nabla V^N(0)}^2}{2} + \frac{L+1}{2} \norm{x}^2,
\end{align*}
where in the second line we use Young's inequality $\langle x,y\rangle \leq \frac{1}{2}\left(\norm{x}^2 + \norm{y}^2\right)$. Now, given that $V^N(0)$ converges to $V(0)$ and as we have show $\norm{\nabla V^N(0)}$ is bounded, we get $C_1=(L+1)/2$ and $C_2 = \sup_{N \in \N} \verts{V^N(0)} + \frac{\norm{\nabla V^N(0)}^2}{2} < + \infty$, which finishes the proof of the second part of the lemma.
\end{proof}

\begin{lemma}\label{lem:rescaling_functionals}
Let $(f_N)_{n\in \N^*}$ be a sequence of continuous functions, $f_N : \R^d \rightarrow \R$. Assume that $f_N$ converge to $f : \R^d \rightarrow \R$, uniformly on compact subsets. Let $(c_N)_{N\in \N^*}$ be a sequence of real numbers, such that $\lim_{N \rightarrow \infty} c_N = c$, where $c \in \R$ is finite. Then $c_N f_N$ converges to $cf$, uniformly on compact subsets. 
\end{lemma}
\begin{proof}
First, since $f_N$ converges to $f$ uniformly on compact subsets, the function $f$ is also continuous. Let $K$ be a compact subset of $\R^d$. Then, we have:
\begin{align*}
    \lim_{N \rightarrow \infty} \sup_{x \in K} \verts{c_N f_N(x) - cf(x)} & \leq \lim_{N \rightarrow \infty} \sup_{x \in K} \verts{c_N f_N(x) - c_N f(x)} + \verts{c_N f(x) - cf(x)} \\
    & \leq \lim_{N \rightarrow \infty} c_N \sup_{x \in K} \verts{f_N(x) - f(x)} + \lim_{N \rightarrow \infty} \verts{c_N - c} \sup_{x \in K} \verts{f(x)} = 0
\end{align*}
where the last inequality follows from $\lim_{N\rightarrow \infty} \sup_{x \in K} \verts{f_N(x) - f(x)} = 0$ and $\lim_{n \rightarrow \infty} \verts{c_N - c} =0$, while $\sup_{x \in K} \verts{f(x)} < +\infty$, because $f$ is continuous and $K$ is compact.
\end{proof}


\begin{lemma} \label{lem:unif_conv_compact_subs}
Assume that $f_N$ is a sequence of continuous functions, $f_N : \R^d \rightarrow \R$.  Assume that for each compact set $K$, each of the functions $f_N$ is Lipschitz continuous with Lipschitz constant $L_N^K$, and for each $K$ we have $\sup_{N \in \N} L_N^K < + \infty$. Assume also, that the sequence of function $f_N$ converges pointwise to a function $f$. Then the sequence of functions $f_N$ converges to $f$ uniformly on compact subsets.
\end{lemma}
\begin{proof}
Let $K$ be a compact subset of $\R^d$. Denote $L^K = \sup_{N \in \N} L_N^K$. We have $L < + \infty$ be assumption, and so funciton $f_N$ are equicontinuous on $K$. Let $x_0 \in K$ be a chosen point. Denote $M = \sup_{N \in \N} \verts{f_N(x_0) - f(x_0)}$, which is finite because $f_N(x_0)$ converges to $f(x_0)$. For each $y \in K, N \in \N$ we have:
\begin{equation*}
    \verts{f_N(y)} \leq \verts{f_N(y) - f_N(x_0)} + \verts{f_N(x_0) - f(x_0)} + \verts{f(x_0)}  \leq  L \text{diam}(K) + M + \verts{f(x_0)},
\end{equation*}
therefore the family $f_N$ is equibounded. It now follows, that $f_N$ converges to $f$ uniformly on $K$. By contradiction, assume that it is not the case. Then there would exists a subsequence $f_{N_k}$ such that $f_{N_k}$ converges to $f$ pointwise, but not uniformly. Since functions $f_{N_k}$ are equicontinuous and equibounded on $K$, from Arzela-Ascoli theorem it follows that there is a further subsequence that converges to some limit uniformly on $K$. But this limit is necesserily $f$, since $f_{N_k}$ converges to $f$ pointwise. This is a contradiction. Therefore it follows, that $f_N$ converges uniformly to $f$ on $K$. Since $K$ was an arbitrary compact subset of $\R^d$, we obtain the thesis.
\end{proof}




%old proof for the data fitting term
\subsection{Proof of \Cref{prop:limiting_functional}}\label{sec:proof_gamma_gonv} 

%\sm{I think we can prove the conditions on $\phi$ necessary for the gamma convergence proof separately from the proof of Gamma convergence. This way we can cover a wider range of activaiton functions}
%\begin{assumptionA}
%The activation function $h$ satisfies \verts{h(\ps{b,x})} \leq c_1 + c_2\norm{b}\norm{x}
%\end{assumptionA}
\sm{I think doing the data fitting lemma for general loss will be hard. We will need to assume something on the growth of derivatives of the loss anyway, to get finite integrals in certain parts of the proof. I propose:}
\begin{assumption}\label{ass:loss_regularity}
The loss $l : \R \times \R \rightarrow \R$ is such that one of the two conditions hold:
\begin{enumerate}
    \item For each $y$, the function $x \mapsto l(y,x)$ is $C^1$ function with $L(y)$-Lipschitz continuous gradient, with $L(y) \leq L_0 + L_1\norm{y}$.
    \item For each $y$, the function $x \mapsto l(y,x)$ is $L(y)$-Lipschitz continuous with $L(y) \leq L_0 + L_1\norm{y}$.
\end{enumerate}
\end{assumption}

\begin{proposition}\label{lem:law_large_nb}\textbf{[Data fitting term]} Let $(x_i,y_i)_{i=1}^{\infty}$ be a sequence of data, such that $\lim_{p \rightarrow \infty} \frac{1}{p} \sum_{i=1}^{p} \delta_{(x_i, y_i)}$ converges in $W_2$ distance to $\pi \in \cP_2(\R^d)$. Let $s \in \{1, 2\}$. Assume that $(\nu^N)_{\N^*}$ is a sequence of probability measures in $\cP^N(\R^{2d})$ that converge to a measure $\nu \in \cP(\R^{2d})$ in $W_s$ distance. Suppose that the activation function satisfies \Cref{ass:activation_function} with constant $s$, and let $l(\cdot, \cdot)$ denote the square loss. Assume that $\lim_{p,N\to \infty}p/N=\alpha \in [0,\infty)$, in the sense that $p$ is a function of $N$ such that $\lim_{N \rightarrow \infty} \frac{p}{N} = \alpha$. We then have the convergence:
\begin{equation*}
  \frac{1}{N}\sum_{i=1}^p \int_{\R^{N\times d}} l\left( y_i, \frac{1}{N}\sum_{j=1}^{N} \phi(\theta_j,z_j, x_i) \right)d\gamma^{\otimes N}(\bz)
 \xrightarrow[p,N\to \infty]{} \alpha \E_{(x,y)\sim \pi} \left[l\left(y, \E_{\substack{\theta\sim \nu \\ z\sim \gamma}} \left[ \phi(\theta,z,x) \right]\right)\right]
\end{equation*}
%\begin{equation}
%    \frac{1}{N}\sum_{i=1}^p \int_{\R^{N\times d}} l\left( y_i, \int \phi(\theta,z, x_i) d\nu_N(\theta) \right)d\gamma^{\otimes N}(\bz) = \int \Psi^N(\theta) d\nu(\theta)
%\end{equation}
%for continuous functions $\Psi^N(\theta)$, such that there exist constants $C_{0, \Psi}, C_{1,\Psi}$ for which $\verts{\Psi^N} \leq C_0 + C_1(\norm{\mu(\theta)}_2^2 + \norm{\sigma(\theta)}_2^2)$ and $\Psi^N$ converge uniformly on compact subsets to a function $\Psi$, for which we have:
%\begin{equation}
%    \int \Psi(\theta) d\nu(\theta) = \alpha \E_{\substack{(x,y)\sim \pi}} \left[ l\left(y, \E_{\substack{\theta\sim \nu \\ z \sim \gamma}} \left[ \phi(\theta,z,x) \right]\right)\right] + \alpha \text{Var}_{z \sim \gamma} \left(\E_{\substack{(x,y) \sim \pi \\ \theta \sim \nu}} \phi(\theta, z , x) \right)\
%\end{equation}
\end{proposition}
\begin{proof}

We first handle the square loss. For, convenience, we denote:
\begin{align*}
    \Phi_{N,i}(\theta, z) & = \frac{1}{N} \sum_{j=1}^{N} \phi(\theta_j, z_j, x_i) \\
    \Psi_{N,i} & = \int \phi(\theta, z, x_i) d\gamma(z) d\nu_N(\theta)  \\
    \Psi_{\infty, i} & = \int \phi(\theta, z, x_i) d\gamma(z) d\nu(\theta) \\
    \Gamma_{N, i} & = \frac{1}{N} \int \Var_{z \sim \gamma}(\phi(\theta, z, x_i)). d\nu_N(\theta)
\end{align*}
Note, that $\Phi_{N,i}$ is a function from $\R^{2Nd} \times \R^{Nd} \rightarrow \R$. If $\theta \in \R^{2Nd}$ is such that $\nu_N = \frac{1}{N} \sum_{j=1}^{N} \theta_j$, then by direct computation we have:
\begin{align}
    \int \Phi_{N, i}(\theta, z) d \gamma^{\otimes N}(z) & = \Psi_{N,i} \\
    \int \Phi_{N,i}^2(\theta, z) d\gamma^{\otimes N}(z) & = \Psi_{N,i}^2 + \Gamma_{N,i}.
\end{align}
Using this notation, by direct expansion of the square, we have:
\begin{equation}
    \left(y_i - \Phi_{N,i}(\theta, z) \right)^2 = \left(y_i - \Psi_{\infty, i}\right)^2 + 2y_i \left(\Psi_{\infty, i} - \Phi_{N,i}(\theta, z) \right) + \Phi_{N_i}(\theta, z)^2 - \Psi_{\infty,i}^2.
\end{equation}
Taking the expectation of the above with respect to $\gamma^{\otimes N}$, we get:
\begin{equation}
    \int \left(y_i - \Phi_{N,i}(\theta, z) \right)^2 d\gamma^{\otimes N}(z) = \left(y_i - \Psi_{\infty, i}\right)^2 + 2y_i \left(\Psi_{\infty,i} - \Psi_{N, i} \right) + \Psi_{N,i}^2 - \Psi_{\infty,i}^2 + \Gamma_{N,i}.
\end{equation}
It is easy t 

%Throughout this proof, we will implicitly treat $p$ as a function of $N$, such that $\lim_{N \rightarrow \infty} p(N) = +\infty$ and  $\lim_{N \rightarrow \infty} \frac{p(N)}{N}= \alpha \in [0, \infty)$. 
%We introduce a sequence of functions:
%\begin{align*}
%    \Psi_N(\theta) &= \frac{1}{p} \sum_{i=1}^p \norm{y_i}^2  + \frac{2}{p} \sum_{i=1}^{p} \int_{\R^{d}} y_i \phi(\theta,z, x_i) d\gamma(z) + \frac{1}{p} \sum_{i=1}^p \int_{\R^{d}} \phi(\theta, z, x_i) \left( \int_{\R^{2d}} \int_{\R^{d}} \phi(\theta', z, x_i)  d\nu_N(\theta') \right) d\gamma(z)
%\end{align*}
%With this notation, a direct expansion of the square and interchange of summation and integration with respect to $\gamma$ shows that the loss part of $\mathcal{F}^N$ can be expressed using the integral of $\Psi_N$ with respect to $\nu_N$:
%\begin{equation*}
%    \frac{1}{N} \sum_{i=1}^p \int_{\R^{N\times d}} l\left( y_i, \int \phi(\theta,z, x_i) \nu_N(d\theta)\right)d\gamma^{\otimes N}(\bz) = \frac{p}{N} \int_{\R^{2d}} \Psi_N(\theta) \nu_N(d\theta)
%\end{equation*}
%We will show, that the functions $\Psi_N(\theta)$ are uniformly upper bounded by function of the form $C_1\norm{\theta}^s + C_0$ and converge uniformly on compact subsets to a function:
%\begin{align*}
    %\Psi(\theta) = \int \int_{\R^{N\times d}} l\left(y_i, \int s(g(\theta, z \right)
    %\Psi(\theta) = \int \norm{y}^2 d\pi(x,y) & + 2\int \int_{\R^{d}} y \phi(\theta,z, x) %d\gamma(z) d\pi(x,y) + \int \int_{\R^{N \times d}} \phi(\theta, z, x) \left( \int_{\R^{d}} \phi(\theta', z, x) d\nu(\theta') \right) d\gamma(z) d\pi(x).
%\end{align*}

%We will prove this for each of the three parts of $\Psi_N$ separately. First, denote $\psi_{N,1}(\theta) = \frac{1}{p} \sum_{i=1}^p \norm{y_i}^2$. We also introduce the notation $\hat{\pi}_N = \frac{1}{p} \sum_{i=1}^p \delta_{(x_i, y_i)}$. Notice that by \Cref{th:villani}:
%\begin{equation*}
%    \lim_{N \rightarrow \infty} \psi_{N,1}(\theta) = \lim_{N \rightarrow \infty} \int \norm{y}^2 d\hat{\pi}_N(x,y) = \int \norm{y}^2 d\pi(x,y),
%\end{equation*}
%since by assumption $\lim_{N \rightarrow \infty} W_2(\hat{\pi}_N, \pi) = 0$.  Therefore $\sup_{p} \frac{1}{p} \sum_{i=1}^p \norm{y_i}^2 < \infty$ \ak{assuming the limit is finite right?}. Therefore the constant function $\psi_{N,1}(\theta)$ is upper bounded by a function of the form $C_1 + C_2 \norm{\theta}^2$ (with $C_2 = 0$), and converges uniformly in $\theta$ to a constant function $\psi_1(\theta) = \int \norm{y}^2 d\pi(x,y)$, as $N,p\rightarrow \infty$.

%For the second part, by  \Cref{ass:activation_function}, we have that for each compact subset $K$ of $\R^{2d}$, there exists a constant $C_K$, such that the function $q(\theta, x_i) = \int_{\R^d} \phi(\theta, z, x_i) d\gamma(z)$ is $C_K\norm{x_i}$-Lipschitz continuous in $\theta$ on the set $K$. Therefore the function:
%\begin{equation*}
%    \psi_{N,2}(\theta) = \frac{1}{p} \sum_{i=1}^{p} \int_{\R^{d}} y_i \phi(\theta,z, x_i) d\gamma(z)
%\end{equation*}
%is $C_K(\frac{1}{p} \sum_{i=1}^p \norm{x_i} \verts{y_i})$-Lipschitz continuous in $\theta$ on the set $K$. By inequality $\verts{ab} \leq \frac{1}{2}(a^2 + b^2)$ for real numbers, the function $\psi_{N,2}$ is Lipschitz-continuous in $\theta$ on the set $K$ with a Lipschitz constant $L^K_N = \frac{C_K}{2}\int \left(\norm{(x,y)}^2 \right) d\hat{\pi}_N(x,y)$. Since $\lim_{N \rightarrow \infty} \int\left( \norm{(x,y)}^2 \right) d\hat{\pi}(x,y) = \int \left( \norm{(x,y)}^2 \right) d\pi(x,y)$, we have that $\sup_{N} L^K_N$ is finite. Therefore by \Cref{lem:unif_conv_compact_subs}, to show uniform convergence on compact subsets we only need to show that the sequence $\phi_{N,2}$ converges pointwise. By  \Cref{ass:activation_function}, we have that 
%\begin{equation*}
%    \norm{\int y\phi(\theta,z , x) d\gamma(z)} \leq C_{q,0}\norm{y} + C_{q,1}\norm{\theta}^2 \norm{x}\norm{y} \leq \left(C_{q,0} + C_{q,1}\norm{\theta}^2 \right) \norm{(x,y)}^2.
%\end{equation*}
%From this it follows that:
%\begin{equation*}
%    \lim_{N \rightarrow \infty} \psi_{N,2}(\theta) = \lim_{N \rightarrow \infty} \int \int_{\R^d} y \phi(\theta, z, x) d\gamma(z) d\hat{\pi}_N(x,y) = \int \int_{\R^d} y\phi(\theta,z,x)d\gamma(z) d\pi(x,y),
%\end{equation*}
%because again, we have $\lim_{N \rightarrow \infty} W_2(\hat{\pi}_N, \pi) = 0$. Therefore the functions $\psi_{N,2}$ converge uniformly on compact subsets to a function $\psi_2$ defined by:
%\begin{equation*}
%    \psi_2(\theta) = \int_{\R^d} y\phi(\theta,z,x)d\gamma(z) d\pi(x,y).
%\end{equation*}

%Now we look at the convergence of sequence of functions $\psi_{N,3}$, defined by:
%\begin{equation*}
%    \psi_{N,3}(\theta) = \frac{1}{p}\sum_{i=1}^p \int_{\R^{d}} \phi(\theta, z, x_i) d\gamma(z) \left( \int_{\R^{2d}} \int_{\R^{d}} \phi(\theta', z, x_i) d\gamma(z) d\nu_N(\theta') \right).
%\end{equation*}
%First, we will argue that for all $i \in \N$, we have:
%\begin{equation}\label{eq:proof_loss_conv1}
%    \sup_{N \in \N} \int_{\R^{2d}} \int_{\R^{d}} \phi(\theta', z, x_i) d\gamma(z) d\nu_N(\theta') \leq \tilde{C}_0 + \tilde{C}_1 \norm{x_i}
%\end{equation}
%where $\tilde{C}_0, \tilde{C}_1$ are constants independent of $\theta'$ and $x_i$. By  \Cref{ass:activation_function}, we have $\norm{\int_{\R^{d}} \phi(\theta', z, x_i) d\gamma(z)} \leq C_{q,0} + C_{q,1}\norm{\theta'}^2 \norm{x_i}$. Since $\nu_N$ converge to $\nu$ in $W_2$ distance, we have that $\lim_{N \rightarrow \infty} \int \norm{\theta'}^2 \nu_N(d\theta') = \int \norm{\theta'}^2 d\nu(\theta')$. From that it follows, that $C' = \sup_{N \in \N} \int \norm{\theta'}^2 d\nu_N(\theta')$ is finite. Therefore for all $N \in \N$, we have:
%\begin{equation*}
%    \norm{ \int_{\R^{2d}} \int_{\R^{d}} \phi(\theta', z, x_i) d\gamma(z) d\nu_N(\theta')} \leq   \int_{\R^{2d}} \norm{\int_{\R^{d}} \phi(\theta', z, x_i) d\gamma(z) }d\nu_N(\theta') \leq C_{q,0} + C_{q,1}C' \norm{x_i},
%\end{equation*}
%and equation \ref{eq:proof_loss_conv1} is satisfied with $C_0 = C_{q,0}$ and $C_1 = C_{q,1}C'$.
%Now, let $K$ be some chosen compact subset of $\R^{2d}$. Recall that the function $\int \phi(\theta, z,x) d\gamma(z)$ is $C_K\norm{x}$-Lipschitz continuous on $K$ by \Cref{ass:activation_function}. Therefore the function $\psi_{N,3}$ is Lipschitz continuous on $K$ with a Lipschitz constant $\tilde{L}^K_N = C_K\frac{1}{p} \sum_{i=1}^p \norm{x_i}(\tilde{C}_0 + \tilde{C}_1\norm{x_i})$. Again, since $\lim_{N \rightarrow \infty} W_2(\hat{\pi}_N, \pi) = 0$, we have that $\sup_{N \in \N} \tilde{L}^K_N$ is finite. Therefore by  \Cref{lem:unif_conv_compact_subs}, in order to show that functions $\psi_{N,3}$ converge uniformly on compact subsets, we only need to show that they converge pointwise. Denote:
%\begin{equation*}
%\end{equation*}

%by the functions $\psi_{N,4} = \frac{1}{p} \sum_{i=1}^p \int_{\R^{d}} \phi(\theta, z, x_i) d\gamma(z)$ are 

%What is left, is identifying the limit, to which $\Psi_N$ converges uniformly on compact subsets. 

\end{proof}



%\begin{lemma}
%Let $(\nu_n)$ be a sequence of probability measures in $\mathcal{P}_2(\R^{2d})$ converging to $\nu \in \mathcal{P}_2(\R^{2d})$ in $W_2$ distance. Assume that for some $\phi: \R^n \rightarrow \R^+$ we have $\phi(x) \leq C_1\norm{x - x_0}_2^2 + C_2$ for some $x_0 \in \R^n$ and $C_1,C_2 \in \R^{+}$. Then $\lim_{n \rightarrow \infty} \int \phi(x) \nu_n(dx) = \int \phi(x) \nu(dx)$.
%\end{lemma}
%\begin{proof}
%Let $r > 0$ be a chosen number, and denote by $B(x_0, r)$ an open ball of radius $r$ centered at $x_0$. Since $W_2$ convergence implies weak convergence (ref), we have:
%\begin{equation*}\label{lem:quad_major_conv_eq1}
%    \lim_{n \rightarrow \infty} \int_{B(x_0,r)} (\norm{x - x_0}_2^2 - r^2) \nu_n(dx) = \int_{B(x_0, r)} (\norm{x-x_0}_2^2 - r^2) \nu(dx)
%\end{equation*}
%because the function $\mathbf{1}_{x \in B(x_0, r)} \left(\norm{x - x_0}_2^2 - r^2\right)$ is continuous and bounded. Furthermore, since $W_2$ convergence implies the convergence of second moments we have $\lim_{n \rightarrow \infty} \int (\norm{x-x_0}_2^2 - r^2) \nu_n(dx) = \int (\norm{x-x_0}_2^2-r^2) \nu(dx)$. Substracting \ref{lem:quad_major_conv_eq1} from this equality, we get: 
%\begin{equation*}    \lim_{n \rightarrow \infty} \int_{B(x_0,r)^c} (\norm{x-x_0}_2^2 - r^2) \nu_n(dx) = \int_{B(x_0,r)^c} (\norm{x-x_0}_2^2 - r^2) \nu(dx)\end{equation*}
%Since $B(x_0,r)$ is a an open set, we have $\liminf_{n \rightarrow \infty} \nu_n(B(x_0, r)) \geq \nu(B(x_0,r))$, and thus $\liminf_{n \rightarrow \infty} \int_{B(x_0, r)} r^2 \nu_n(dx) \geq \int_{B(x_0,r)} \nu(dx)$. Therefore we have:
%\end{proof}



 %where $\psi_N$ is defined in \Cref{lem:law_large_nb}. 

%By \Cref{lem:V_1}, both $\alpha V_1$ and $\nicefrac{1}{p}V_2^N$ have Lipschitz gradients\ak{check how the second constant depends on $N$ if it's the case}, hence $\exists {c_1,c_2}$ such that $\int \alpha V_1(\theta)d\nu(\theta), \int \nicefrac{1}{p}V_2^N(\theta)\le c_1 \int \|\theta\|^2 d\nu(\theta) + c_2$.

%Then, the second term in \eqref{eq:v1_composite} can be written:
%\begin{align*}
%  \int_{\R^{d}} \log\prior(w)dq(w|\theta)&=\frac{1}{(2\pi)^{d/2} \prod_{k=1}^d \sigma_{jk}}  \int_{\R^d} \log\left(\frac{1}{(2\pi)^{d/2}\tsigma^2}\exp\left(-\frac{\| w\|^2}{2\tsigma^2}\right)\right) \exp\left(-\frac{(w-\mu)^T \Sigma^{-1}(w-\mu)}{2\sigma^2}\right)dw\\
%  &= \frac{1}{(2\pi)^{d/2}\prod_{k=1}^d \sigma_{k}} \int_{\R^d} \left(- d\log  \tsigma_{k} - \frac{\|z\|^2}{2} -\frac{d}{2} \log(2\pi)\right)\exp\left(-\frac{\|z\|^2}{2}\right)\prod_{k=1}^d \sigma_{k} dz \\
%\end{align*}s(
%\end{proof}




\begin{proposition}\label{prop:gamma_convergence_bnn}
Assume that data $(x_i,y_i)$ are sampled i.i.d. from a distribution $\pi \in \mathcal{P}_2(\R^d)$. Then with probability one the sequence $(\cF^{N})$ $\Gamma$-converges to $\cF$ and we have a limit of minimizers and minimums.
\end{proposition}

\begin{proof}
(1) Let $\nu \in \cP_2(\R^{2d})$ and let $\nu^N\to \nu$ in the $W_2$ sense. For $N\ge 0$, if $\nu^N$ is not in the domain of $\cF^N$, then $\cF^{N}(\nu^N)=+\infty$ and \eqref{eq:upp_bound_gamma} holds. Otherwise, if for all $N\ge 0$, $\nu^N$ is in the domain of $\cF^N$, by \Cref{lem:law_large_nb}, $\lim_{N\to \infty} \cF^{N}(\nu^{N})=\cF(\nu)$\ak{cite Lemma 10}, either in regime 1 or regime 2, by \Cref{prop:scale_prior_variance} in the latter. In both cases \eqref{eq:upp_bound_gamma} holds.


(2) Let $\nu \in \cP_2(\R^{2d})$. Consider the empirical measure $\bar{\nu}^N=\frac{1}{N}\sum_{j=1}^N \delta_{\theta_j}$ where $\theta_1,\dots,\theta_N$ are i.i.d. samples of $\nu$. Almost surely,  $W_2(\bar{\nu}^N,\nu)\to 0$
(see \citep[Proposition 2.2.6]{panaretos2020invitation}). Then, for any $N\ge 0$, $\bar{\nu}^N$ is finitely supported and is in the domain of $\cF^{N}$. By \Cref{lem:law_large_nb}, $\cF(\nu)=\lim_{N\to \infty} \cF^{N}(\bar{\nu}^{N})$.
\end{proof}


\section{Auxiliary results}\label{sec:auxiliary_results}


%\begin{remark} \label{rem:ass_activ_func_quadbound}
%A direct consequence of \Cref{ass:activation_function} is that the function $q(\theta, x) = \int \phi(\theta,z,x) d\gamma(z)$ satisfies the bound $\norm{q(\theta,x)} \leq C_{q,0} + C_{q,1} \norm{\theta}^2 \norm{x}$, with $C_{q,0} = C_{\phi,0}$ and $C_{q,1} = C_{\phi,1} \int \norm{z}^r d\gamma(z)$.
%\end{remark}


\begin{lemma}\label{lem:relU_and_sigmoid}
\Cref{ass:activation_function}-(i) and (ii) with $s=2$ is satisfied for a Lipschitz activation function $h$.
\Cref{ass:activation_function}-(ii) with $s=1$ is satisfy only if the output weights of the neural network are fixed and bounded, or if the activation $h$ is bounded. 
\end{lemma}

\subsection{Proof of \Cref{lem:relU_and_sigmoid} }\label{sec:proof_relU_and_sigmoid}
\begin{proof} Recall that if $h$ is the RelU: $ u \mapsto \max(0,u)$ or sigmoid: $u \mapsto (1+\exp(-u))^{-1}$ activation function, then it is 1-Lipschitz.

1.
We will show that the function $\theta \mapsto \phi(\theta, z, x)$ is Lipschitz continuous in $\theta$ on each compact set as soon as . Remember, that 
\begin{equation*}
\phi(\theta, z, x) = s(g(\theta, z), x) = s(w,x)= a h(\ps{b,x}),\text{ where } w=(a,b)=g(\theta,z) = \mu + \log(1+\exp(\rho))\odot z,
\end{equation*}
where $\rho \mapsto \log(1+\exp(\rho))$ is $1$-Lipschitz. 
For $z\in \R^d$, we firstly have for $w,w'\in \R^d$
\begin{multline*}
    \|w-w'\| = \|g(\theta,z)-g(\theta',z)\| = \|\mu-\mu' + (\log(1+\exp(\rho))-\log(1+\exp(\rho')))\odot z \|\\
    \le \|\mu-\mu'\| + \|\rho-\rho'\|\|z\| \le \|\theta - \theta'\|(1+\|z\|),
\end{multline*}
and $\|w\|=\|g(\theta,z)\| \le \|\mu\|+\|\log(1+\exp(\rho)\|\|z\| \le \|\theta\|(1+\|z\|)$.

Hence, for $z,x\in \R^d\times \X$, for $\theta,\theta'\in \R^{2d}$, by denoting $w=g(\theta,z)=(a,b)$ and $w'=g(\theta',z)=(a',b')$, and using the Lipschitzness of the activation functions, we have:
\begin{multline*}
    \|\phi(\theta,z,x)-\phi(\theta',z,x)\| = \|a h(\ps{b,x})-a' h(\ps{b',x})\| = \|(a-a')h(\ps{b,x}) + a'(h(\ps{b,x})-h(\ps{b',x}))\| \\
    \le \|a-a'\| |h(\ps{b,x})| + \|a'\||h(\ps{b,x})-h(\ps{b',x})|\le \|a-a'\|\|b\| \|x\| + \|a'\| \|b-b'\|\|x\|\\\le \|w-w'\|.\|x\|(\|w\|+\|w'\|)
    \le \|\theta-\theta'\|(1+\|z\|)^2 \|x\| (\|\theta\|+\|\theta'\|).
\end{multline*}
 Hence, for each compact set $K$ of $\R^{2d}$, there exists $c_K>0$ such that $\|\theta\|+\|\theta'\|\le C_K$, hence for any $x\in \X$
%\begin{equation*}
%   \|q(\theta,x)-\phi(\theta',x)\|= \|\int_{\R^d}\phi(\theta,z,x)-\phi(\theta',z,x)d\gamma(z)\|\le \|x\| \|\theta-\theta'\| c_K \left\Vert\int (1+\|z\|)^2d\gamma(z)\right\Vert := C_K \|x\| \|\theta-\theta'\|,
%\end{equation*}
\begin{equation*}
   \|\phi(\theta,z,x)-\phi(\theta',z,x)\|\le C_K  \|x\|(1+\|z\|)^2 \|\theta-\theta'\|,
\end{equation*}
and \Cref{ass:activation_function}-(i) holds.


2. We have for any $\theta,z,x\in \R^{2d}\times \R^{d}\times \X$:
\begin{equation*}
     \| \phi(\theta,z,x)\| = \|a h(\ps{b,x})\|\le \|a\||h(\ps{b,x}|.%\le \|g(\theta,z)\|^2\|x\|  \le (\|\mu\|+\|\sigma\| \|z\|)^2 \|z\|    \le 2 (\|\mu\|^2 + \|\sigma\|^2 \|z\|^2) \|x\|.
\end{equation*}
where $w=(a,b)=g(\theta,z)=\mu + \log(1+\exp(\rho))\odot z$, where $\|g(\theta,z)\| \le \|\mu\| + \|\rho\|.\|z\|\le \|\theta\|(1+\|z\|)$ since $\rho\mapsto \log(1+\exp(\rho))$ is $1$-Lipschitz. We now consider  three cases.

\textit{First case.} We assume $h$ is $L$-Lipschitz for $L>0$. Then,
\begin{equation*}
    \| \phi(\theta,z,x)\| \le \|a\| L \|b\|\|x\| \le L\|g(\theta,z)\|^2 \|x\|\le L \|\theta\|^2(1+\|z\|)^2 \|x\|,
\end{equation*}
hence \Cref{ass:activation_function}-(ii) is verified with $s=2$.


\textit{Second case.} If $h$ is bounded by $H>0$. Then 
\begin{equation*}
    \| \phi(\theta,z,x)\| \le \|a\| H \le \|g(\theta,z)\| H \le H (1+\|z\|)\|\theta\|.
\end{equation*}

\textit{Third case.} We assume $h$ is Lipschitz (not necessarily bounded) but also the output weights are fixed and bounded by some constant $A>0$. Then
\begin{equation*}
    \|\phi(\theta,z,x)\|\le A \|b\|\|x\| \le A \|g(\theta,z)\|\|z\| \le A \|x\| (1+\|z\|) \|\theta\|
\end{equation*}
hence \Cref{ass:activation_function}-(ii) is verified with $s=1$.

%Hence,
%\begin{equation*}
%    \|\int \phi(\theta,z,x)d\gamma(z)\| \le 2 \int \|z\|^2 d\gamma(z) (\|\mu\|^2 +\|\sigma\|^2)\|x\|:=C_{\phi} (\|\mu\|^2+\|\sigma\|^2)\|x\|.
%\end{equation*}
%\end{proof}


\subsection{Proof of \Cref{lem:V_Lipschitz}}\label{sec:proof_V_Lipschitz}
\begin{proof}
Recall that $\prior=\cN(\mu',\diag(\tau^2))$ and $\tq(w|\theta):=\mathcal{N}(\mu,\diag(\log(1+\exp(\rho))^2))$ with $\tau=(\tau_1,\dots,\tau_d),\rho=(\rho_1,\dots,\rho_d) \in \R^d$. Then,
\begin{equation}\label{eq:v1_composite}
    V(\theta)=\frac{1}{2}\left[ \sum\limits_{k=1}^d \left( -2 \log\left(\frac{\log\left(1+\exp(\rho_k)\right)}{\tau_k^2}\right)+\frac{\log(1+\exp(\rho_k))^2}{\tau_k^2} + \frac{(\mu_k-\mu'_k)^2}{\tau_k^2} \right) - d \right]
\end{equation}
%\begin{equation}
%    V(\theta)= \KL(\tq(\cdot|\theta)|\prior)= \int_{\R^{d}} \log\left( \frac{\tq(w|\theta)}{\prior(w)}\right)d\tq(w|\theta)= \int_{\R^{d}} \log \tq(w|\theta)d\tq(w|\theta) - \int_{\R^{d}} \log\prior(w)d\tq(w|\theta).
%\end{equation}
% Since $\log \prior(w) = C - \frac{\Vert w \Vert^2}{2\tau^2}$, the second term in \eqref{eq:v1_composite} can be identified as minus half the variance of $q(w | \theta)$, plus the constant $C$ independent of $\theta$. The gradient of the second term with respect to $\theta$ is  therefore equal to:
%\begin{align}
%    \nabla_{\theta}\left(  \frac{1}{2\tau^2} \sum_{k=1}^d \sigma^2_{k}\right) = \nabla_{\theta}\left( \frac{1}{2\tau^2} \sum_{k=1}^d \log(1 + \exp(\rho_{k}))^2\right).
%\end{align}

To establish the claim, we will show that $\nabla V$ is Lipschitz. We now treat each term separately.

The second derivative of $f:\rho \mapsto \log(1+\exp(\rho))^2$ is bounded. Indeed, we have
\begin{equation*}
    f''(\rho)=\frac{2\exp(\rho)}{(1+\exp(\rho)^2)}\left( \exp(\rho) +\log(1+\exp(\rho)\right).
\end{equation*}
Hence, $f''$ is continuous and $\lim_{\rho\to \infty}f''(\rho)=1$, $\lim_{\rho\to - \infty}f''(\rho)=0$; hence it is bounded and $f'$ is Lipschitz continuous.
%We have established the Lipschitz continuity of the gradient of the second term in \eqref{eq:v1_composite}.

%\begin{align}
%    \nabla_{\theta} \frac{1}{2} \sum_{j=1}^N \sum_{k=1}^d \sigma_{j,k} = \nabla_{\theta} \frac{1}{2} \sum_{j=1}^d\sum_{k=1}^d \log(1 + \exp(\rho_{j,k})).
%\end{align}
%It is easy to see, that to establish that Lipschitz continuity of the above function with a constant independent of $d, N$ is implied by Lipschitz continuity of the derivative of $f(t) = \log(1 + \exp(t))$. Since the derivative of $f$ is the standard logistic function: $\nicefrac{d}{dt} \log(1 + \exp(t)) = \nicefrac{\exp(t)}{1 + \exp(t)}$, 
%we have established the Lipschitz continuity of the gradient of the second term in \eqref{eq:v1_composite}.

%On the other hand, the first term in \eqref{eq:v1_composite} can be rewritten:
%\begin{align*}
%   & \int_{\R^{d}} \log q(w|\theta)dq(w|\theta)\\
%    &= \frac{1}{(2\pi)^{d/2} \prod_{k=1}^d \sigma_{k}} \int_{\R^{d}} \log \left(\frac{\exp\left(-\frac{( w-\mu)^T\Sigma^{-1}(w-\mu)}{2\sigma^2}\right)}{(2\pi)^{d/2}\prod_{k=1}^d \sigma_{k}} \right) \exp\left(-\frac{(w-\mu)\Sigma^{-1}(w-\mu)}{2\sigma^2}\right)dw \\
%    &= \frac{1}{(2\pi)^{d/2}\prod_{k=1}^d \sigma_{k}} \int_{\R^d} \left(- \sum_{k=1}^{d}\log  \sigma_{k} - \frac{\|z\|^2}{2} -\frac{d}{2} \log(2\pi)\right)\exp\left(-\frac{\|z\|^2}{2}\right)\prod_{k=1}^d \sigma_{k} dz \\
%    & =\frac{1}{(2\pi)^{d/2} } \int_{\R^d} \left(- \sum_{k=1}^{d}\log  \sigma_{k} -\frac{\|z\|^2}{2}-\frac{d}{2} \log(2\pi)\right)\exp\left(-\frac{\|z\|^2}{2}\right)\ dz \\
%    &= \cH(\gamma) -\sum_{k=1}^{d}\log  \sigma_{jk} = \cH(\gamma)-\sum_{k=1}^{d}\log\left(\log\left(1+\exp(\rho_{k})\right)\right).
%\end{align*}
%where $\cH(\gamma)=\int_{\R^d}\log(\gamma(z))d\gamma(z)$ is the negative entropy of $\gamma$.

%Again, to show that the gradient of the above expression with respect to $\theta$ is Lipschitz continuous with a constant independent of $d,N$, it is enough to show that the derivative of $g(\rho) = \log(\log(1+ \exp(\rho)))$ is Lipschitz continuous. To prove it, we will show that the second derivative of $g$ is bounded.

We now deal with $g: \rho\mapsto \log(\log(1+\exp(\rho)))$. Through routine calculations, we obtain:
\begin{equation*}
    g'(\rho) = \frac{1}{\log(1+\exp(\rho))} \cdot \frac{\exp(\rho)}{1 + \exp(\rho)}, \quad 
    g''(\rho) =  -\left( g'(\rho) \right)^2 + \frac{g'(\rho)}{1+\exp(\rho)}.
\end{equation*}
Notice, that as $\rho \rightarrow \infty$, then $g'(\rho) \rightarrow 0$, and hence $g''(\rho) \rightarrow 0$ as well. On the other hand, when $\rho \rightarrow -\infty$, we have $\exp(\rho) \rightarrow 0$ and thus 
\[
\lim_{\rho \rightarrow -\infty} \frac{\exp(\rho)}{\log(1+\exp(\rho))} = \lim_{\rho \rightarrow -\infty} \frac{\exp(\rho) - 0}{\log(1+\exp(\rho)) - 0} = 1,
\]
since the derivative of $\log(1+x)$ at $x=0$ is equal to $1$. This means that $\lim_{\rho \rightarrow -\infty} g'(\rho) = 1$, and hence $\lim_{\rho\rightarrow -\infty} g''(t) = 0$. Since the second derivative of $g$ is continuous and vanishes at infinity, it is bounded. Hence $g'$ is Lipschitz continuous. %which concludes our proof.

The last non-constant term involves the function $\mu \mapsto (\mu-\mu')^2$ which, similarly, has bounded second derivative.

Combining the above, there exists $L>0$ such that $\nabla V$ is $L$-Lipschitz. Then, by using the L-smoothness inequality:
\begin{equation*}
    |V(\theta)|\le |V(0)|+\ps{\nabla V(0), \theta} +\frac{L}{2}\|\theta\|^2 \le |V(0)|+\frac{\|\nabla V(0)\|^2}{2}+\frac{L+1}{2}\|\theta\|^2,
\end{equation*}
by using Young's inequality $\ps{a,b}\le \frac{1}{2}(\|a\|^2+\|b\|^2)$. Hence, there exists $C_V^0,C_V^1>0$, such that
\begin{equation*}
    \int V(\theta)d\nu(\theta)\le C_V^0+C_V^1 \|\theta\|^2.\qedhere
\end{equation*}
\end{proof}


%\begin{lemma} \label{lem:unif_lip_cont_regime2_reg}
%Let $C$ be a positive constant, and let
%\begin{equation*}    f_C(\rho) = C^2 \left(-\log\left(\frac{\log(1+\exp(\rho + C))^2}{C^2}\right) + \frac{\log(1+\exp(\rho + C))^2}{C^2} - 1 \right),
%\end{equation*}
%then $f_C(\rho)$ has Lipschitz-continuous gradients with a Lipschitz constant independent of $C$.
%\end{lemma}


%\ak{below: for equicoerciveness of the
%$V_2^N$}
%\begin{lemma}
%Lef $s \in \R$ be a constant. Let $f(t) = \frac{\log(1 + \exp(t + \rho)}{t}$, $g(x) = -\log(x) + x - 1$. Then the function $h(t) = tg(f(t))$ is:
%\begin{itemize}
%    \item increasing on $(0,\infty)$ for $s \geq 0$
%    \item ??? for $s < 0$
%\end{itemize}
%\end{lemma}
%\begin{proof}
%Assume that $s \geq 0$. The first derivative of $f$ is given by
%\begin{equation*}
%    \frac{d}{dt}f(t) = \frac{\frac{\exp(t+s)}{1+\exp(t+s)}\cdot t - \log(1 + \exp(t+s))}{t^2}.
%\end{equation*}
%Since 
%\end{proof}

\begin{lemma}
Suppose that $\prior=\cN(\mu', \diag(\tau^2))$, $\tilde{q}(.|\theta)=\cN(\mu, \diag(\sigma^2))$ where $\sigma = \log(1+\exp(\rho))$. Then there exist constants $C_1 \ge 0$, $C_0 \le 0$, such that $V_1(\theta) \geq C_1( \norm{\mu(\theta)}^2 + \norm{\sigma(\theta)}_2^2) + C_0$.
\end{lemma}
\begin{proof}
Remember, that we have:
\begin{equation*}
V_1(\theta) = \frac{1}{2}\left[ \sum\limits_{k=1}^d \left(\log\left(\frac{\tau^2_k}{\sigma^2_k}\right) +\frac{\sigma^2_k}{\tau^2_k} +\frac{ (\mu_k-\mu'_k)^2}{\tau^2_k} \right) - d \right].
\end{equation*}
Denote $\taumax = \max\limits_{1 \leq k \leq d} \tau_k$ and $\taumin = \min\limits_{1 \leq k \leq d} \tau_k$. For any two real numbers $a,b$ the inequality $(a +b)^2 \leq 2a^2 + 2b^2$ holds. Therefore
\begin{equation*}
    \verts{\mu_k}^2 \leq 2\verts{\mu_k - \mu_k'}^2 + 2\verts{\mu_k'}^2,
\end{equation*}
from which it follows that
\begin{equation}\label{eq:V1_quad_lower_bound_mu}
    \sum\limits_{k=1}^d \frac{\|\mu_k - \mu_k'\|^2}{\tau_k^2} \geq \sum\limits_{k=1}^d \left(\frac{\verts{\mu_k}^2}{2\tau_k^2} - \frac{\verts{\mu_k'}^2}{\tau_k^2} \right) \geq \frac{\norm{\mu(\theta)}^2}{2\taumax^2} - \frac{\norm{\mu'}_2^2}{\taumin^2}.
\end{equation}
For the variance part, we will use the $-\log(x) \geq 1 - x$ inequality which works for $x > 0$. This inequality is a simple rewriting of the well known $\log(1+x) \leq x$. We have:
\begin{equation*}
    \log\left(\frac{\tau^2_k}{\sigma^2_k}\right) = - \log\left(\frac{\sigma^2_k}{2\tau^2_k}\right) - \log(2) \geq \frac{\sigma^2_k}{2\tau^2_k} + 1 - \log(2).
\end{equation*}
From the above it follows, that 
\begin{equation} \label{eq:V1_quad_lower_bound_sigma}
    \frac{1}{2}\left[ \sum\limits_{k=1}^d \left(\log\left(\frac{\tau^2_k}{\sigma^2_k}\right) +\frac{\sigma^2_k}{\tau^2_k} \right) \right] \geq \frac{\norm{\sigma(\theta)}^2}{2\taumax^2} + d(1 - \log(2)).
\end{equation}
Combining \ref{eq:V1_quad_lower_bound_mu} and \ref{eq:V1_quad_lower_bound_sigma}, we get:
\begin{equation*}
    V_1(\theta) \geq \frac{1}{2\taumax^2} \left( \norm{\mu(\theta)}_2^2 + \norm{\sigma(\theta)}_2^2 \right) - d\log(2) - \frac{\norm{\mu'}_2^2}{\taumin^2}
\end{equation*}
which concludes the proof.
\end{proof}

%\begin{lemma}
%Then there exists a constant $C_1'>0, C_0' < 0$ such that $V_1(\theta) \ge C_1'( \norm{\mu} + \|\rho\| + C_0'.$
%\end{lemma}\begin{proof}\begin{equation*}   V_1(\theta)=\frac{1}{2} \sum\limits_{k=1}^d \left( -2 \log\left(\frac{\log\left(1+\exp(\rho_k)\right)}{\tau^2}\right)+\frac{\log(1+\exp(\rho_k))^2}{\tau^2} + \frac{(\mu_k-\mu'_k)^2}{\tau^2} \right)\end{equation*}\end{proof}


==> checklist.tex <==
\section*{Checklist}



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    (total amount of compute: unknown, type of ressource: internal cluster with GPUs)
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

